Revisiting Network Support for RDMA

The advent of RoCE (RDMA over Converged Ethernet) has led to a significant increase in the use of RDMA in datacenter networks. To achieve good performance, RoCE requires a lossless network which is in turn achieved by enabling Priority Flow Control (PFC) within the network. However, PFC brings with it a host of problems such as head-of-the-line blocking, congestion spreading, and occasional deadlocks. Rather than seek to fix these issues, we instead ask: is PFC fundamentally required to support RDMA over Ethernet? We show that the need for PFC is an artifact of current RoCE NIC designs rather than a fundamental requirement. We propose an improved RoCE NIC (IRN) design that makes a few simple changes to the RoCE NIC for better handling of packet losses. We show that IRN (without PFC) outperforms RoCE (with PFC) by 6-83% for typical network scenarios. Thus not only does IRN eliminate the need for PFC, it improves performance in the process! We further show that the changes that IRN introduces can be implemented with modest overheads of about 3-10% to NIC resources. Based on our results, we argue that research and industry should rethink the current trajectory of network support for RDMA.

==> iwarp.tex <==
\section{Comparison with iWARP}
\label{sec:iwarp-vs-irn}
%\paragraphb{IRN vs iWARP:} 
%\fixme{Alex: we don't really know how iWarp is implemented, besides that they use TCP-like transport, and we cannot estimate how close they are to optimal network performance. We have lab results showing that they perform noticeably worse, even compared to current ConnectX-4 RoCE: \url{http://www.mellanox.com/related-docs/whitepapers/WP_RoCE_vs_iWARP.pdf} }
\eat{As mentioned before, we believe that iWARP had the right architecture (allowing the NICs to deal with losses more efficiently rather than making the network lossless), but RoCE NICs were considered to be simpler and more mature (being based largely on what was used for Infiniband). IRN adopts an architecture closer to iWARP (where the NIC implements better loss recovery), but with an implementation closer to RoCE (carefully limiting the functionality on the NIC to basic building blocks, rather than embodying the entire transport stack).} 

IRN is similar to iWARP in that it explicitly handles losses (borrowing elements of TCP as discussed in \S\ref{sec:irnTransportDesign}), but its design is closer to RoCE's, with an emphasis on simplicity. iWARP and IRN have very different underlying philosophies: iWARP was designed to support RDMA over TCP in hardware, making as little changes to the TCP stack as possible. It requires multiple layers to translate RDMA's segments into TCP's bytes, along with subtle changes to RDMA's application semantics to support these layers. IRN's design philosophy, on the other hand, is to support efficient loss recovery for traditional Infiniband-based RDMA, making as little changes to it as possible. IRN works directly on RDMA segments. Moreover, it exclusively targets datacenter networks, exploiting their properties (such as small BDP) to ease state management. As a result, IRN's implementation is simpler than iWARP: compare $<$600 lines of C++ code for IRN's transport logic synthesized on an FPGA device using $<$4\% resources (\S\ref{sec:fpgaSynthesis}), with the significantly larger code-base for the TCP stack requiring years of effort by hardware experts and careful pipelining to sustain required message rates, when realized on iWARP NICs~\cite{intelPersonal}.


\begin{figure}[t]
\centering
 \renewcommand{\arraystretch}{0.1}
 \footnotesize

\renewcommand{\arraystretch}{1.0}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ccc}


 \begin{subfigure}
 \centering
\includegraphics[width=0.1\textwidth,height=0.12\textwidth]{figures/irn-vs-iwarp/graph-iwarp-vs-irn-avgSlowdown.pdf}
 \end{subfigure} 
 
 &
 
  \begin{subfigure}
\centering
\includegraphics[width=0.1\textwidth,height=0.12\textwidth]{figures/irn-vs-iwarp/graph-iwarp-vs-irn-avgFCT.pdf}
\end{subfigure}

&

\begin{subfigure}
\centering
\includegraphics[width=0.1\textwidth,height=0.12\textwidth]{figures/irn-vs-iwarp/graph-iwarp-vs-irn-tailFCT.pdf}
\end{subfigure}


%congestion control & congestion control

\end{tabular}

\caption{The figures compares iWARP's transport (TCP stack) with IRN (without explicit congestion control) using three metrics (average slowdown, average FCT and 99\%ile FCT).}

\vspace{-10pt}
\label{fig:irn-vs-iwarp}
\end{figure}

One question that remains though, is whether IRN's simplicity over the TCP stack implemented in iWARP impacts performance? We, thus, compared, via simulations, IRN's performance with full-blown TCP stack's, using INET simulator's in-built TCP implementation for the latter. Figure~\ref{fig:irn-vs-iwarp} shows the results for the default scenario. We find that absence of slow-start (with use of BDP-FC instead) results in 21\% smaller slowdowns with IRN and comparable average and tail FCTs. These results show that in spite of a simpler design, IRN's performance is better than full-blown TCP stack's, even without any explicit congestion control. Augmenting IRN with TCP's AIMD logic further improves its performance, resulting in 44\% smaller average slowdown and 11\% smaller average FCT as compared to iWARP. 

%\fixme{an alternative to having a separate section for this is to put the result in \S\ref{sec:deepDive} and the first paragraph in \S\ref{sec:discussion}. What do you think is more readable?}
